Towards Robust Toxic Content Classification

Toxic content detection aims to identify content that can offend or harm its recipients. Automated classifiers of toxic content need to be robust against adversaries who deliberately try to bypass filters. We propose a method of generating realistic model-agnostic attacks using a lexicon of toxic tokens, which attempts to mislead toxicity classifiers by diluting the toxicity signal either by obfuscating toxic tokens through character-level perturbations, or by injecting non-toxic distractor tokens. We show that these realistic attacks reduce the detection recall of state-of-the-art neural toxicity detectors, including those using ELMo and BERT, by more than 50% in some cases. We explore two approaches for defending against such attacks. First, we examine the effect of training on synthetically noised data. Second, we propose the Contextual Denoising Autoencoder (CDAE): a method for learning robust representations that uses character-level and contextual information to denoise perturbed tokens. We show that the two approaches are complementary, improving robustness to both character-level perturbations and distractors, recovering a considerable portion of the lost accuracy. Finally, we analyze the robustness characteristics of the most competitive methods and outline practical considerations for improving toxicity detectors.

==> TableDetailedMerged.tex <==

\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{@{}lll|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Model} &
\multicolumn{1}{l}{\multirow{2}{*}{Train Noise}} & \multicolumn{1}{l|}{\multirow{2}{*}{Test Noise}} & \multicolumn{3}{c}{Jigsaw 2018} & \multicolumn{3}{|c}{OffensEval 2019} \\ \cmidrule(l){4-9} 
& &  & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{|c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} \\ \midrule
%%%%%% BERT %%%%%%
\multirow{10}{*}{BERT} &
%& \multicolumn{1}{l}{} & \multicolumn{6}{c}{BERT} \\ \midrule
None & C & 0.911 & 0.600 & 0.608 & 0.757 & 0.446 & 0.313 \\
 & &  & -6.44\% & -12.34\% & -33.46\% & -14.87\% & -38.85\% & -56.65\% \\
&C & C & 0.922 & 0.588 & 0.697 & 0.783 & 0.618 & 0.529 \\
& &  & -5.37\% & -14.04\% & -23.81\% & -11.97\% & -15.34\% & -26.58\% \\
&None & D & \textbf{0.970} & \textbf{0.682} & \textbf{0.882} & \textbf{0.881} & \textbf{0.705} & 0.650 \\
& &  & -0.47\% & -0.41\% & -3.56\% & -0.97\% & -3.49\% & -9.83\% \\
&D & D & \textbf{0.971} & \textbf{0.683} & \textbf{0.904} & \textbf{0.885} & \textbf{0.714} & 0.650 \\
& &  & -0.33\% & -0.20\% & -1.10\% & -0.50\% & -2.21\% & -9.83\% \\
&C + D & None & \textbf{0.968} & \textbf{0.653} & 0.904 & \textbf{0.875} & \textbf{0.685} & \textbf{0.739} \\
& &  & -0.59\% & -4.60\% & -1.08\% & -1.64\% & -6.16\% & -11.49\% \\ \midrule 
 %%%%%% CDAE %%%%%%
\multirow{10}{*}{CDAE}% & \multicolumn{1}{l}{} & \multicolumn{6}{c}{CDAE (ours)} \\ \midrule
&None & C & \textbf{0.925} & \textbf{0.610} & \textbf{0.642} & \textbf{0.758} & \textbf{0.465} & \textbf{0.354} \\
& &  & -4.90\% & -9.87\% & -28.17\% & -11.92\% & -30.19\% & -52.24\% \\
&C & C & \textbf{0.932} & \textbf{0.596} & \textbf{0.706} & \textbf{0.786} & \textbf{0.629} & \textbf{0.533} \\
& &  & -4.18\% & -11.99\% & -21.00\% & -8.72\% & -5.47\% & -28.01\% \\
&None & D & 0.965 & 0.669 & 0.810 & 0.864 & 0.672 & \textbf{0.708} \\
& &  & -0.75\% & -1.20\% & -9.40\% & 0.36\% & 0.98\% & -4.50\% \\
&D & D & 0.970 & 0.672 & 0.882 & 0.862 & 0.691 & \textbf{0.683} \\
& &  & -0.25\% & -0.74\% & -1.39\% & 0.15\% & 3.78\% & -7.87\% \\
&C + D & None & \textbf{0.968} & 0.651 & \textbf{0.912} & 0.858 & 0.655 & 0.721 \\
& &  & -0.54\% & -3.84\% & 2.01\% & -0.35\% & -1.50\% & -2.81\% \\ 
 
%  \midrule
%  & \multicolumn{1}{l}{} & \multicolumn{6}{c}{BERT+CDAE} \\ \midrule 
% None & C + D & 0.921 & 0.590 & 0.725 & 0.774 & 0.505 & 0.404 \\
%  & & -5.35\% & -12.26\% & -20.65\% & -12.75\% & -30.57\% & -44.25\% \\
% C + D & C + D & 0.942 & 0.628 & 0.799 & 0.827 & 0.612 & 0.604 \\
%  &  & -3.17\% & -6.45\% & -12.53\% & -6.87\% & -15.92\% & -16.66\% \\ 
 \bottomrule
\end{tabular}
\caption{\label{tab:detresults_merge} Detailed Results for the CDAE and BERT (Percentages below are changes relative to the unnoised baseline). C refers to character-level perturbations and D refers to distractors. Numbers in \textbf{bold} are best results for each setting/metric. Adversarial training helps most against character-level perturbations.  The CDAE is stronger against character-level perturbations, whereas BERT performs well in the presence of distractors. \an{Maybe change all the percentages to one decimal digit? They are too distracting. Single decimal will still get the point across}}
\end{center}
\end{table*}


\iffalse
% Please add the following required packages to your document preamble:
\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{@{}lll|rrr|rrr@{}}
\toprule
\multirow{2}{*}{Model} &
\multicolumn{1}{l}{\multirow{2}{*}{Train Noise}} & \multicolumn{1}{l|}{\multirow{2}{*}{Test Noise}} & \multicolumn{3}{c}{Jigsaw 2018} & \multicolumn{3}{|c}{OffensEval 2019} \\ \cmidrule(l){4-9} 
& &  & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{|c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} \\ \midrule
%%%%%% BERT %%%%%%
\multirow{10}{*}{BERT} &
%& \multicolumn{1}{l}{} & \multicolumn{6}{c}{BERT} \\ \midrule
None & C & 0.911 & 0.600 & 0.608 & 0.757 & 0.446 & 0.313 \\
& &  & -6.44\% & -12.34\% & -33.46\% & -14.87\% & -38.85\% & -56.65\% \\
&C & C & 0.922 & 0.588 & 0.697 & 0.783 & 0.618 & 0.529 \\
& &  & -5.37\% & -14.04\% & -23.81\% & -11.97\% & -15.34\% & -26.58\% \\
&None & D & \textbf{0.970} & \textbf{0.682} & \textbf{0.882} & \textbf{0.881} & \textbf{0.705} & 0.650 \\
& &  & -0.47\% & -0.41\% & -3.56\% & -0.97\% & -3.49\% & -9.83\% \\
&D & D & \textbf{0.971} & \textbf{0.683} & \textbf{0.904} & \textbf{0.885} & \textbf{0.714} & 0.650 \\
& &  & -0.33\% & -0.20\% & -1.10\% & -0.50\% & -2.21\% & -9.83\% \\
&C + D & None & \textbf{0.968} & \textbf{0.653} & 0.904 & \textbf{0.875} & \textbf{0.685} & \textbf{0.739} \\
& &  & -0.59\% & -4.60\% & -1.08\% & -1.64\% & -6.16\% & -11.49\% \\ \midrule 
 %%%%%% CDAE %%%%%%
\multirow{10}{*}{CDAE}% & \multicolumn{1}{l}{} & \multicolumn{6}{c}{CDAE (ours)} \\ \midrule
&None & C & \textbf{0.925} & \textbf{0.610} & \textbf{0.642} & \textbf{0.758} & \textbf{0.465} & \textbf{0.354} \\
& &  & -4.90\% & -9.87\% & -28.17\% & -11.92\% & -30.19\% & -52.24\% \\
&C & C & \textbf{0.932} & \textbf{0.596} & \textbf{0.706} & \textbf{0.786} & \textbf{0.629} & \textbf{0.533} \\
& &  & -4.18\% & -11.99\% & -21.00\% & -8.72\% & -5.47\% & -28.01\% \\
&None & D & 0.965 & 0.669 & 0.810 & 0.864 & 0.672 & \textbf{0.708} \\
& &  & -0.75\% & -1.20\% & -9.40\% & 0.36\% & 0.98\% & -4.50\% \\
&D & D & 0.970 & 0.672 & 0.882 & 0.862 & 0.691 & \textbf{0.683} \\
& &  & -0.25\% & -0.74\% & -1.39\% & 0.15\% & 3.78\% & -7.87\% \\
&C + D & None & \textbf{0.968} & 0.651 & \textbf{0.912} & 0.858 & 0.655 & 0.721 \\
& &  & -0.54\% & -3.84\% & 2.01\% & -0.35\% & -1.50\% & -2.81\% \\ 
 
%  \midrule
%  & \multicolumn{1}{l}{} & \multicolumn{6}{c}{BERT+CDAE} \\ \midrule 
% None & C + D & 0.921 & 0.590 & 0.725 & 0.774 & 0.505 & 0.404 \\
%  & & -5.35\% & -12.26\% & -20.65\% & -12.75\% & -30.57\% & -44.25\% \\
% C + D & C + D & 0.942 & 0.628 & 0.799 & 0.827 & 0.612 & 0.604 \\
%  &  & -3.17\% & -6.45\% & -12.53\% & -6.87\% & -15.92\% & -16.66\% \\ 
 \bottomrule
\end{tabular}
\caption{\label{tab:detresults_merge} Detailed Results for the CDAE and BERT (Percentages below are changes relative to the unnoised baseline). C refers to character-level perturbations and D refers to distractors. Numbers in bold are best results for each setting/metric. Adversarial training helps most against character-level perturbations.  The CDAE is stronger against character-level perturbations, whereas BERT performs well in the presence of distractors.}
\end{center}
\end{table*}
\fi

==> TableEnsemble.tex <==
\begin{table*}[t]
\small
\begin{center}
\begin{tabular}{cccccccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{Train Noise}} & \multicolumn{1}{l|}{\multirow{2}{*}{Test Noise}} & \multicolumn{3}{c}{Jigsaw 2018} & \multicolumn{3}{|c}{OffensEval 2019} \\ \cmidrule(l){3-8} 
\multicolumn{1}{l}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{|c}{AUC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Recall} \\ 
\midrule
None & C + D & 0.921 & 0.590 & 0.725 & 0.774 & 0.505 & 0.404 \\
%  & & -5.35\% & -12.26\% & -20.65\% & -12.75\% & -30.57\% & -44.25\% \\
C + D & C + D & 0.942 & 0.628 & 0.799 & 0.827 & 0.612 & 0.604 \\
%  &  & -3.17\% & -6.45\% & -12.53\% & -6.87\% & -15.92\% & -16.66\% \\ 
\bottomrule
\end{tabular}
\end{center}
\caption{ \label{tab:ensemble} Results of the Ensemble of CDAE and BERT. The ensemble performs the strongest against combined noise among all of our methods. \ab{I would repeat BERT and CDAE results here too. Otherwise the reader would have to rummage though a bunch of tables to confirm our conclusions.} \an{Good idea. You have space; do it} }
\end{table*}

==> noise_effect_results.tex <==
\begin{table}[t]
\small
\begin{center}
\begin{tabular}{l|rr|rr}
\toprule
\multicolumn{1}{l|}{\multirow{2}{*}{Noise}} & \multicolumn{2}{c}{Jigsaw 2018} & \multicolumn{2}{|c}{OffensEval 2019} \\ 
\multicolumn{1}{l|}{} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{\% Change} & \multicolumn{1}{|c}{Recall} & \multicolumn{1}{c}{\% Change} \\ \midrule
 & \multicolumn{4}{c}{BERT-based model} \\ \midrule
None &  0.914 &  & 0.721 & \\
C &  0.918 & -33.40 & 0.313 & -56.65 \\
D & 0.882 & -3.47 &  0.650 & -9.83 \\
C+D & 0.604 & -33.92 &  0.342 & -52.57 \\
\midrule
 & \multicolumn{4}{c}{CDAE-based model (ours)} \\ 
 \midrule
 None &  0.894 & & 0.721 & \\
C &  0.642 & -28.17 & 0.354 & -52.24 \\
D & 0.810 & -9.40 &  0.708 & -4.50 \\
C+D & 0.597 & -33.22 &  0.388 & -46.19 \\
 \bottomrule
\end{tabular}
\caption{\label{tab:noised_results} Effect of Noise on BERT and CDAE based models. Overall, recall decreases substantially under adversarial attacks. Character noise has a stronger effect than distractors on both models.}
\end{center}
\end{table}
